The continuing search for evidence of tidal orbital decay of hot Jupiters

Many of the known hot Jupiters are formally unstable to tidal orbital decay. The only hot Jupiter for which orbital decay has been directly detected is WASP-12, for which transit timing measurements spanning more than a decade have revealed that the orbital period is decreasing at a rate of $dP/dt\approx 10^{-9}$, corresponding to a reduced tidal quality factor of about $2\times 10^5$. Here, we present a compilation of transit-timing data for WASP-12 and eleven other systems which are especially favorable for detecting orbital decay: KELT-16; WASP-18, 19, 43, 72, 103, 114, and 122; HAT-P-23; HATS-18; and OGLE-TR-56. For most of these systems we present new data that extend the time baseline over which observations have been performed. None of the systems besides WASP-12 displays convincing evidence for period changes, with typical upper limits on $dP/dt$ on the order of $10^{-9}$ or $10^{-10}$, and lower limits on the reduced tidal quality factor on the order of $10^5$. One possible exception is WASP-19, which shows a statistically significant trend, although it may be a spurious effect of starspot activity. Further observations are encouraged.

==> REFREP <==
Prof. Joshua N. Winn
Princeton University
Peyton Hall, 4 Ivy Lane
Princeton, NJ 08540
(609) 258-4342
jnwinn@princeton.edu

Dear Dr. Endl,

Thank you for organizing the review of our manuscript, "The Apparently
Decaying Orbit of WASP-12."  We appreciate the referee's very prompt
report.  We have carefully considered the corrections and suggestions
in the report and have prepared a revised manuscript.  Below, we
reproduce the report along with our responses.

Thank you for your further consideration.

Sincerely,

Josh Winn

---------------------------

In this paper, the authors present an analysis of new and published
transit and occultation timing measurements of the hot Jupiter WASP-12
b. They detect a significant deviation from a linear ephemeris, which
they interpret as being due to either orbital decay or apsidal
precession, although they are unable to definitively distinguish
between these two models. The existence of both of these effects for
hot Jupiters is a long-standing theoretical prediction, and as the
first real observational confirmation of (one of) these predictions
this work is suitable for publication in the Astronomical Journal once
a few concerns have been addressed. The paper is well-written and
thorough, and my concerns about the paper as currently written are
mostly minor. I have included my comments and concerns below, in order
of appearance in the paper.

-----

Title: 

-"The Apparently Decaying Orbit of WASP-12" Technically, this should
 be WASP-12b. WASP-12 is the star, WASP-12b the planet; it is the
 orbit of the planet that is decaying.

   Changed as suggested.

Section 1: 

-"WASP-12b is one of the shortest-period giant planets known" Please
 quote the period.

   Changed as suggested.  

Section 2: 

-Fig. 1 caption: please explicitly note that each transit light curve
 is offset vertically for clarity.

   Changed as suggested.  

-If there is an instrument paper describing KeplerCam, please cite it
 here (it is not obvious from a quick ADS search that such a paper
 exists, however).

   We are not aware of any such publication.

-It seems to me that something is missing in the description of the
 transit model. The three parameters Rp/R*, R*/a, and b are sufficient
 to fix the transit shape, but not the time scale of the transit,
 i.e., the transit duration (cf. Eqn. 3 of Seager & Mallen-Ornelas
 2003, ApJ, 585, 1038). How did the authors handle this? Did they
 assume some constant period, or determine the time scale from their
 fit parameters, Kepler's third law, and the stellar mass, or use some
 other method? Please clarify.

   The period was held fixed, as explained in the revised paragraph.
   
-Please specify which set of stellar parameters were used to find the
 limb-darkening values (presumably those from the Hebb et
 al. discovery paper for WASP-12b?).

   They were indeed the parameters from Hebb et al. (2009), as now
   stated in the revised text.

-When citing Foreman-Mackey et al., please include the name of the
 MCMC code (emcee).

   Changed as suggested.  

-Are the values for Rp/R*, R*/a, b, etc. found by the MCMC fits
 generally consistent with published values of these parameters?

   Yes, as noted in a sentence that has been added to the 2nd-to-last
   paragraph of Sec. 2.
   
Section 3:

-From the text of this section and Fig. 2, the provenance of the 3.6
 versus 4.5 micron Spitzer data is unclear. Was one occultation
 observed in each band? If so, does each panel in Fig. 2 represent
 data from a single new occultation, or does Fig. 2 also show the
 reanalyzed data from Deming et al. (2015)? Please clarify.

  One occultation was observed in each band, as now explained in the
  first paragraph of Sec. 3.  Fig. 2 only shows the new data; the
  revised caption gives the epoch numbers.

-I suggest quoting how many occultations were observed by Deming et
 al. (2015), and reanalyzed by the authors, in the main text
 (currently this is only able to be determined by counting the number
 of appearances of footnote "b" in Table 1).

  The first paragraph of Sec. 3 now states that 2 new occultation
  times were measured, and one occultation dataset was reanalyzed.

-The procedures used to derive the Spitzer photometry are described in
 much greater detail than those used for the KeplerCam photometry in
 Section 2. I suggest going into more detail in Section 2 to match
 Section 3 (e.g., quote aperture sizes, any detrending applied, etc.)

  The detrending is described (a linear function of airmass). The
  revised paper also gives the target S/N and choice of aperture
  radius.

-It would be helpful to the reader to include a brief (~1-2 sentence)
 definition of the "noise pixel radius." Please provide a citation for
 the Allan deviation relation and/or provide a brief description of
 how this is defined.

  Changed as suggested.  A footnote was added to describe the Allan
  deviation relation.  We also took the opportunity to correct an
  error in our original manuscript: the individual exposure times were
  2.0 seconds and not 0.4 second.
  
-Which version of the Spitzer photometry did the authors adopt for
 each occultation, and how close did they come to achieving the
 theoretical photon noise limit? Were there any significant
 differences in the values of t_o found from the different methods
 used on the same data? What bin length for the time-binned data
 turned out to be most optimal?

  All this information is now provided in the revised paragraphs.

Section 4:

-As far as I could tell, the variable E (epoch number) is never
 defined. Please explicitly define this variable in the text, as it is
 not in as standard usage as variables like t, P, etc.

  E is now defined after Eqn. (3).

-The authors use both t_0 (reference epoch) and t_o (time of
 occultation) as variables, sometimes in the same equation (Eqns. 3,
 5, 8). The similarity of the characters 0 and o could cause
 confusion. I suggest changing t_o to t_occ (and t_t to t_tra to
 match), as these are the abbreviations used for transits and
 occultations, respectively, in Table 1.

   Changed as suggested.  

-"Our new data--the square points at the rightmost extreme of the
 plot--follow the trend that had been established by the prior data."
 It is not clear whether this is referring to the trend found by
 Maciejewski et al. (2016), or if the authors fit the literature data
 separately before adding in their new data for the final fit. Please
 clarify.

   We replaced "the prior data" with "Maciejewski et al. (2016)".

-By eye in Fig. 3, it appears that the preference for the decay model
 is largely driven by the single transit measurement from the 2008
 season, from Hebb et al. as analyzed by Maciejewski et al. What are
 the Delta chi squared/Delta AIC/Delta BIC values between the models
 if this single datapoint is excluded? If this datapoint is simply a
 statistical outlier, what impact would this have on the conclusions?
 Additionally, there appears to be some confusion about the original
 time standard of these data (see Footnote 5 of Maciejewski et
 al. 2013); can the authors exclude an incorrect time standard being
 used for these data as the source of the large timing residual for
 this transit?

  When the data are refitted without that data point, \Delta\chi^2 is
  reduced from 5.5 to 2.0.  This is now noted at the end of Sec. 4. We
  do not have any more information than Maciejewski et al. (2013)
  about that particular data point.  
  
Section 5.1:

-While P/(dP/dt) is straightforward to calculate, the time until P
 shrinks to 0 is not particularly physically meaningful; in reality,
 the planet will be destroyed before this time. I suggest instead
 calculating and quoting the time until either the planet reaches the
 Roche limit, or until it impacts the stellar surface. Obviously the
 process of tidal disruption is more complicated than captured in such
 a calculation, but I think this would be a more accurate estimate of
 the remaining lifetime of the planet.

  Since this is meant to be an order of magnitude calculation, we
  prefer leaving the text as it is.  The actual time evolution of a(t)
  is more complicated because Q may vary with period, Roche lobe
  overflow might be stable or unstable, etc.

-The rate of period decay is denoted as Pdot in the abstract and dP/dt
 in the main text (except for quoting the period derivative due to the
 Shklovskii effect in Section 5.4). Please use consistent notation.

  We prefer to leave it as it is, because Pdot is more easily read
  within a line of text.  There is little danger of confusion.

Section 5.3: 

-Are the tidal decay and apsidal precession models mutually exclusive,
 i.e., could both processes be operating simultaneously? Or does
 e.g. the strength of tidal dissipation necessary to induce measurable
 orbital decay also imply that the eccentricity should be too low for
 apsidal precession to be measurable? I do not think that fitting a
 combined model would be useful given the number of free parameters,
 but this could be worth clarification.

  The models are not mutually exclusive, as now mentioned in Sec. 5.4.

-When mentioning that there are no other known planets in the WASP-12
 system, please provide a reference for this statement (probably
 Knutson et al. 2014, which the authors already cite in the next
 section).

  Changed as suggested.

-If there is some mechanism that can excite a low level of
 eccentricity for hot Jupiters, and it also operates in other systems,
 should apsidal precession be (relatively) common for hot Jupiters?
 Are there other particular systems for which a search for apsidal
 precession (or orbital decay) should be undertaken in order to
 constrain this possibility?

  Because the mechanism is unknown, no clear recommendations can be
  given.  Indeed upon reflection we are uncomfortable citing the
  particular explanation of Phinney (1992) in the abstract; we have
  omitted that sentence, although we preserved the discussion in
  Sec. 5.2.

-A general comment regarding this section: it is perhaps notable that
 WASP-12 has among the highest values of R*/a and Rp/a among giant
 planets (rivaled or exceeded only by WASP-103b and WASP-19b,
 respectively), and since the expected tidal decay and precession
 rates are proportional to these parameters to the fifth power, it is
 perhaps unsurprising that these effects should be detected first for
 WASP-12b.

  The promising qualities of WASP-12 are described in the
  introduction.

Section 5.4: 

-It is not clear why the authors do a rough calculation to find that
 the period derivative due to the Shklovskii effect is ~10^-14, and
 then in the next sentence do a more precise calculation to find that
 Pdot~6x10^-15. Quoting one or the other number would be sufficient.

  Indeed this was an oversight. The sentence has been changed.

-Presumably the limits on acceleration of the system and additional
 bodies in the system from Knutson et al. 2014, also rule out the
 period change being due to transit timing variations caused by either
 light travel time effects or dynamical interactions between WASP-12b
 and a second planet?

  Yes. We clarified Sec. 5.4 by adding the phrase "due to the force
  from companion stars or wide-orbiting planets."

Section 6: 

-The authors mention that one of the other notable properties of
 WASP-12 b is that its orbital plane may be misaligned with respect to
 the stellar rotation. One of the postulates of the tidal realignment
 hypothesis to describe the distribution of spin-orbit misalignments
 as a function of stellar effective temperature is that tides should
 be able to realign hot Jupiters without destroying them through
 orbital decay (e.g., Winn et al. 2010, Rogers & Lin 2013, Li & Winn
 2016). In this framework, it seems strange that WASP-12 b should be
 experiencing significant orbital decay, but still possess a
 misaligned orbit. Could the authors comment upon this point?

  We prefer not to enter into this discussion because it would take
  several paragraphs to treat this subject properly, and there is
  little/nothing that can be concluded at this stage. Observationally,
  the spin-orbit misalignment has not been securely demonstrated.
  Theoretically, the relationship between tidal realignment and
  orbital decay is not clear; for example there may be dissipation
  mechanisms that lead to realignment without decay (Lai et al. 2012,
  MNRAS, 423, 486).
  
Table 1:

-Typo in table heading: "Epoch numnber"

  Corrected.

Table 2:

-Values related to omega are here quoted in terms of radians, but
 omega dot is quoted in terms of degrees in the text. Please use
 consistent units.

  We prefer to leave the text as it is. Some readers may want to know
  the answer in deg/year, others may want to know in rad/epoch.  In
  performing our analysis we found both sets of units to be useful.

-------------------------------------------------------------------------

Comment from Statistics Editor:

A comment on language around equation 1:

a) Eqn 1 is a weighted least squares statistic, not a likelihood
function. Unweighted LS and MLE give the same result (by theorem)
under some conditions, but this is not generally for weighted LS.

  We changed the terminology to that of Foreman-Mackey et al. (2013):
  "The transition distribution was proportional to $\exp(-\chi^2/2)$
  with..."

b) The previous sentence mentions priors: but there is no Bayesian
inference here. MCMC is a capable algorithm that has no special
attachment to Bayesian calculations .. it can be used for least
squares calculations as well.

  We removed this sentence.

c) I suggest giving a different designation to the statistic in eqn 1
(perhaps X^2), as it is chi-squared distributed only under specific
conditions.

  We prefer to leave it as it is, because in our experience \chi^2 is
  a frequently used symbol for the sum-of-squares of the residuals.


==> abs <==
We present new transit and occultation times for the hot Jupiter
WASP-12b. The data are compatible with a constant period derivative:
$\dot{P}=-29 \pm 3$~ms~yr$^{-1}$ and $P/\dot{P}= 3.2$~Myr. However, it
is difficult to tell whether we have observed orbital decay, or a
portion of a 14-year apsidal precession cycle. If interpreted as
decay, the star's tidal quality parameter $Q_\star$ is about $2\times
10^5$. If interpreted as precession, the planet's Love number is
$0.44\pm 0.10$. Orbital decay appears to be the more parsimonious
model: it is favored by $\Delta\chi^2=5.5$ despite having two fewer
free parameters than the precession model. The decay model requires
the unlikely coincidence that WASP-12 was discovered within the final
$\sim$0.2\% of its existence, but this harmonizes with independent
evidence that the planet is nearing disruption. Precession does not
invoke any temporal coincidence, but only if some unknown mechanism is
maintaining an eccentricity of $\approx$0.002 in the face of rapid
tidal circularization. A speculative possibility is Phinney's (1992)
theory of eccentricity excitation by gravitational perturbations from
the star's convective eddies. To distinguish unequivocally between
decay and precession will probably require a few more years of
monitoring. Particularly helpful will be occultation timing in 2019
and thereafter.

